Evaluation of a Simple, Scalable, Parallel Best-First Search Strategy

Large-scale, parallel clusters composed of commodity processors are increasingly available, enabling the use of vast processing capabilities and distributed RAM to solve hard search problems. We investigate Hash-Distributed A* (HDA*), a simple approach to parallel best-first search that asynchronously distributes and schedules work among processors based on a hash function of the search state. We use this approach to parallelize the A* algorithm in an optimal sequential version of the Fast Downward planner, as well as a 24-puzzle solver. The scaling behavior of HDA* is evaluated experimentally on a shared memory, multicore machine with 8 cores, a cluster of commodity machines using up to 64 cores, and large-scale high-performance clusters, using up to 2400 processors. We show that this approach scales well, allowing the effective utilization of large amounts of distributed memory to optimally solve problems which require terabytes of RAM. We also compare HDA* to Transposition-table Driven Scheduling (TDS), a hash-based parallelization of IDA*, and show that, in planning, HDA* significantly outperforms TDS. A simple hybrid which combines HDA* and TDS to exploit strengths of both algorithms is proposed and evaluated.

==> ability.tex <==
\begin{table}
\caption{Comparison of the number of problems solved}
\begin{center}
{\tiny
\begin{tabular}{|c||c|c|c|c||c|}
\hline
\# of CPU Cores             &    1  &   16    &   64  &  128  & Number of \\
(Total memory size (GB))    &  (16) &  (32)   & (128) & (256) & Test Problems \\
\hline
\hline
Depot                       &    7  &    7    &    7     &       7  & 22\\
\hline
Drivers log                 &   11  &   11    &   11     & {\bf 12} & 20\\
\hline
Freecell                    &    5 &  {\bf 6} &  {\bf 7} &  {\bf 7} & 20\\
\hline
Rovers                      &    7 &     7    &  {\bf 8} &  {\bf 8} & 20\\
\hline
Satellite                   &    6 &     6    &  {\bf 7} &  {\bf 7} & 20 \\
\hline
Zeno travel                 &    9 &     9    & {\bf 10} & {\bf 10} & 20 \\
\hline
Pipes world (no tankage)    &   18 &    18    & {\bf 19} & {\bf 19} & 19 \\
\hline
Pegsol                      &   27 & {\bf 28} & {\bf 29} & {\bf 29} & 30 \\
\hline
Sokoban                     &   11 & {\bf 16} & {\bf 20} & {\bf 21} & 30 \\
\hline
\end{tabular}
}
\end{center}
\end{table}

==> fungate_results_aij_final.tex <==
Speedups (1-8 cores)
            & 1 core & HDA*(4 cores)       & PRA*(4 cores)       & WSA* (4 cores)      & HDA* (8 cores)       & PRA* (8 cores)     & WSA* (8 cores)      & Abst. time & Opt. plan Len.
Depot4      & 73.34  & 29.70 (2.47, 0.62)  & 39.07 (1.88, 0.47)  & 34.12 (2.15, 0.54)  & 15.79 (4.64, 0.58)  & 21.18 (3.46, 0.43)  & 19.40 (3.78, 0.47)  &  3.56 & 30 
\hline
Driverlog8  & 85.79  & 39.72 (2.16, 0.54)  & 56.57 (1.52, 0.38)  & 48.94 (1.75, 0.44)  & 20.74 (4.14, 0.52)  & 34.03 (2.52, 0.32)  & 30.21 (2.84, 0.35)  &  0.15 & 22 
\hline
Freecell5   & 143.57 & 47.41 (3.03, 0.76)  & 56.24 (2.55, 0.64)  & 52.32 (2.74, 0.69)  & 24.90 (5.77, 0.72)  & 30.84 (4.66, 0.58)  & 27.67 (5.19, 0.65)  &  8.17 & 30 
\hline
Rover12     & 517.67 & 221.61 (2.34, 0.58) & 286.31 (1.81, 0.45) & 256.31 (2.02, 0.50) & 117.27 (4.41, 0.55) & 162.18 (3.19, 0.40) & 145.90 (3.55, 0.44) &  1.03 & 19 
\hline
ZenoTrav9   & 170.61 & 75.65 (2.26, 0.56)  & 113.96 (1.50, 0.37) & 92.82 (1.84, 0.46)  & 40.90 (4.17, 0.52)  & 66.61 (2.56, 0.32)  & 57.99 (2.94, 0.37)  &  0.19 & 21 
\hline
PipesNoTk14 & 201.52 & 71.79 (2.81, 0.70)  & 96.90 (2.08, 0.52)  & 87.60 (2.30, 0.58)  & 38.23 (5.27, 0.66)  & 58.35 (3.45, 0.43)  & 53.69 (3.75, 0.47)  &  1.70 & 30 
\hline
PipesTk15   & 81.26  & 27.19 (2.99, 0.75)  & 36.83 (2.21, 0.55)  & 32.59 (2.49, 0.62)  & 15.00 (5.42, 0.68)  & 21.02 (3.87, 0.48)  & 19.03 (4.27, 0.53)  &  7.31 & 30 
\hline
Pegsol28    & 837.78 & 269.10 (3.11, 0.78) & 370.04 (2.26, 0.57) & 335.10 (2.50, 0.63) & 138.47 (6.05, 0.76) & 233.29 (3.59, 0.45) & 215.04 (3.90, 0.49) &  0.64 & 35 
\hline
Sokoban22   & 474.75 & 149.46 (3.18, 0.79) & 195.49 (2.43, 0.61) & 180.50 (2.63, 0.66) & 77.82 (6.10, 0.76)  & 115.80 (4.10, 0.51) & 106.60 (4.45, 0.56) &  2.23 & 172 
\hline



==> speedup.tex <==
\begin{table*}
\caption{Execution time and speedup for hard problems (Abstraction size = 1000)}
\begin{tabular}{|c||c|c|c|c||c|}
\hline
\# of CPU Cores &	1	&	16	&	64	&	128	& Abstraction time \\ 
\hline
\hline
Depot-13 &	 325.74 &  38.23 (8.52) &  11.86 (27.46) &  10.28 (31.70) &   5.59 \\ 
\hline
Freecell-6 &	   n/a &   n/a (n/a) &	 309.37 (n/a) & 191.09 (n/a) &   n/a \\ 
\hline
Freecell-7 &	   n/a & 246.57 (n/a) &  76.45 (n/a) &  57.82 (n/a) &   n/a \\ 
\hline
Rover-6 &	4373.37 &   n/a (n/a) &	 137.27 (31.86) &   XXX n/a (n/a) HANG XXX &	   0.14 \\ 
\hline
Rover-12 &	 521.13 &  58.09 (8.97) &  16.09 (32.38) &  10.01 (52.04) &   0.20 \\ 
\hline
Satellite-7 &	   n/a &   n/a (n/a) &	 525.99 (n/a) & 297.76 (n/a) &   n/a \\ 
\hline
ZenoTravel-11 &	2688.93 &   n/a (n/a) &	  82.41 (32.63) &  44.90 (59.88) &   0.40 \\ 
\hline
Pipes-No-Tank-24 &	1269.16 & 165.59 (7.66) &  42.27 (30.03) &  34.20 (37.11) &   7.26 \\ 
\hline
Pegsol-28 &	 886.01 &  75.69 (11.71) &  21.75 (40.73) &  17.54 (50.51) &   0.99 \\ 
\hline
Pegsol-29 &	4509.22 &   n/a (n/a) &	 109.65 (41.13) &  75.35 (59.84) &  15.15 \\ 
\hline
Sokoban-12 &	 466.90 &  37.47 (12.46) &  14.24 (32.80) &  12.37 (37.75) &   2.39 \\ 
\hline
Sokoban-14 &	2201.76 &   n/a (n/a) &	  55.75 (39.50) &  34.48 (63.86) &   1.34 \\ 
\hline
Sokoban-15 &	2639.30 &   n/a (n/a) &	  76.55 (34.48) &  45.15 (58.46) &   2.77 \\ 
\hline
Sokoban-16 &	   n/a &   n/a (n/a) &	 162.20 (n/a) &  88.50 (n/a) &   n/a \\ 
\hline
Sokoban-18 &	   n/a &   n/a (n/a) &	  64.69 (n/a) &  38.78 (n/a) &   n/a \\ 
\hline
Sokoban-21 &	1529.45 & 145.76 (10.49) &  45.74 (33.44) &  29.25 (52.28) &   3.77 \\ 
\hline
Sokoban-23 &	 589.89 &  45.89 (12.85) &  16.26 (36.28) &  13.23 (44.60) &   2.06 \\ 
\hline
Sokoban-24 &	 950.55 &  76.82 (12.37) &  26.11 (36.41) &  18.06 (52.62) &   2.37 \\ 
\hline
Sokoban-29 &	   n/a &   n/a (n/a) &	  87.98 (n/a) &  52.22 (n/a) &   n/a \\ 
\hline
Sokoban-30 &	 378.30 &  31.49 (12.01) &  13.05 (29.00) &  11.91 (31.78) &   2.20 \\ 
\hline

\end{tabular}
\end{table*}

==> tsubame_results_aij_final.tex <==
Speedups (16-1024 cores)
            & 1 core  & 16 cores (1 node)    & 64 cores (4 nodes)   & 128 cores (8 nodes)  & 512 cores (32 nodes) & 1012 cores (64 nodes) & Abst. init. time & Opt. plan Len.
Driverlog13 & n/a     & n/a (n/a, n/a)       & n/a (n/a, n/a)       & n/a (n/a, n/a)       & 41.01 (n/a, n/a)     & 27.43 (n/a, n/a)      &  0.63            & 26 
\hline
Freecell6   & n/a     & n/a (n/a, n/a)       & n/a (n/a, n/a)       & 137.08 (n/a, n/a)    & 50.36 (n/a, n/a)     & 23.39 (n/a, n/a)      &  8.45            & 34 
\hline
Freecell7   & 2864.64 & n/a                  & 66.85 (42.85, 0.67)  & 34.00 (84.25, 0.66)  & 11.59 (247.16, 0.48) & 18.92 (151.41, 0.15)  &  10.52           & 41 
\hline
Rover12     & 1149.74 & 109.62 (10.49, 0.66) & 17.68 (65.03, 1.02)  & 14.50 (79.29, 0.62)  & 4.06 (283.19, 0.55)  & 3.47 (331.34, 0.32)   &  0.17            & 19 
\hline
Satellite7  & n/a     & n/a (n/a, n/a)       & 502.51 (n/a, n/a)    & 209.73 (n/a, n/a)    & 55.31 (n/a, n/a)     & 37.64 (n/a, n/a)      &  0.34            & 21 
\hline
ZenoTrav11  & 546.67  & 61.26 (8.92, 0.56)   & 16.58 (32.97, 0.52)  & 8.55 (63.94, 0.50)   & 2.76 (198.07, 0.39)  & 9.05 (60.41, 0.06)    &  0.35            & 14 
\hline
ZenoTrav12  & n/a     & n/a (n/a, n/a)       & n/a (n/a, n/a)       & n/a (n/a, n/a)       & 180.80 (n/a, n/a)    & 90.14 (n/a, n/a)      &  0.48            & 21 
\hline
PipesNoTk24 & 1396.29 & 139.25 (10.03, 0.63) & 40.34 (34.61, 0.54)  & 20.47 (68.21, 0.53)  & 6.11 (228.52, 0.45)  & 11.60 (120.37, 0.12)  &  7.24            & 24 
\hline
Pegsol28    & 1010.65 & 83.22 (12.14, 0.76)  & 21.77 (46.42, 0.73)  & 10.41 (97.08, 0.76)  & 3.23 (312.90, 0.61)  & 2.93 (344.93, 0.34)   &  1.04            & 35 
\hline
Pegsol29    & 5143.24 & n/a                  &  n/a                 & 52.28 (98.38, 0.77)  & 13.86 (371.09, 0.72) & 7.89 (651.87, 0.64)   & 16.76            & 37 
\hline
Pegsol30    & n/a     & n/a (n/a, n/a)       & n/a (n/a, n/a)       & n/a (n/a, n/a)       & 34.14 (n/a, n/a)     & 18.19 (n/a, n/a)      &  3.30            & 48 
\hline
Sokoban24   & 2635.37 & n/a                  & 57.29 (46.00, 0.72)  & 33.52 (78.62, 0.61)  & 15.97 (165.02, 0.32) & 47.91 (55.01, 0.05)   &  1.55            & 205 
\hline
Sokoban26   & n/a     & n/a (n/a, n/a)       & 155.20 (n/a, n/a)    & 77.60 (n/a, n/a)     & 25.29 (n/a, n/a)     & 26.50 (n/a, n/a)      &  2.34            & 135 
\hline
Sokoban27   & n/a     & n/a (n/a, n/a)       & n/a (n/a, n/a)       & n/a (n/a, n/a)       & 36.53 (n/a, n/a)     & 26.57 (n/a, n/a)      &  3.68            & 87 
\hline

Search Overhead (16-1024 cores)
            & 1 core        & 16 cores (1 node)  & 64 cores (4 nodes)  & 128 cores (8 nodes) & 512 cores (32 nodes) & 1024 cores (64 nodes) & Opt. plan Len.
Driverlog13 & n/a (-)       & n/a (n/a)          & n/a (n/a)           & n/a (n/a)           & 625188136 (n/a)      & 854934383 (n/a)       &  26 
\hline
Freecell6   & n/a (-)       & n/a (n/a)          & n/a (n/a)           & 337534088 (n/a)     & 512715407 (n/a)      & 395891702 (n/a)       &  34 
\hline
Freecell7   & 92584775 (-)  & n/a (n/a)          & 94375606 (1.93\%)   & 95500727 (3.15\%)   & 117518741 (26.93\%)  & 211389417 (128.32\%)  &  41 
\hline
Rover12     & 37243958 (-)  & 37307482 (0.17\%)  & 23230170 (-37.63\%) & 37443936 (0.54\%)   & 37561310 (0.85\%)    & 35435932 (-4.85\%)    &  19 
\hline
Satellite7  & n/a (-)       & n/a (n/a)          & 222759213 (n/a)     & 191082376 (n/a)     & 187116616 (n/a)      & 258191728 (n/a)       &  21 
\hline
ZenoTrav11  & 14619024 (-)  & 14619585 (0.00\%)  & 14637721 (0.13\%)   & 14740958 (0.83\%)   & 15724503 (7.56\%)    & 92010559 (529.39\%)   &  14 
\hline
ZenoTrav12  & n/a (-)       & n/a (n/a)          & n/a (n/a)           & n/a (n/a)           & 1185737053 (n/a)     & 1180345571 (n/a)      &  21 
\hline
PipesNoTk24 & 72782203 (-)  & 72805219 (0.03\%)  & 72836410 (0.07\%)   & 73260029 (0.66\%)   & 75243695 (3.38\%)    & 221345652 (204.12\%)  &  24 
\hline
Pegsol28    & 111419815 (-) & 114198633 (2.49\%) & 113524270 (1.89\%)  & 114337541 (2.62\%)  & 118067547 (5.97\%)   & 149248317 (33.95\%)   &  35 
\hline
Pegsol29    & 478930258 (-) & n/a (n/a)          & n/a (n/a)           & 499041168 (4.20\%)  & 501172298 (4.64\%)   & 526933156 (10.02\%)   &  37 
\hline
Pegsol30    & n/a (-)       & n/a (n/a)          & n/a (n/a)           & n/a (n/a)           & 1405030332 (n/a)     & 1421281828 (n/a)      &  48 
\hline
Sokoban24   & 241797086 (-) & n/a (n/a)          & 278360621 (15.12\%) & 356505847 (47.44\%) & 597653466 (147.17\%) & 1504666496 (522.28\%) &  205 
\hline
Sokoban26   & n/a (-)       & n/a (n/a)          & 720848950 (n/a)     & 760380596 (n/a)     & 973650946 (n/a)      & 1388184527 (n/a)      &  135 
\hline
Sokoban27   & n/a (-)       & n/a (n/a)          & n/a (n/a)           & n/a (n/a)           & 1359144655 (n/a)     & 1650729633 (n/a)      &  87 
\hline


Speedups (64 cores, without dummy processes) 
            & 1 core  & 64 cores (4 nodes)   & 64 cores (8 nodes)   & 64 cores (16 nodes)  & 64 cores (32 nodes)   & 64 cores (64 nodes)  & Opt. plan Len.
Freecell7   & 2864.64 & 66.85 (42.85, 0.67)  & 68.61 (41.75, 0.65)  & 64.29 (44.56, 0.70)  & 59.24 (48.36, 0.76)   & 59.39 (48.23, 0.75)  &  41 
\hline
Rover12     & 1149.74 & 17.68 (65.03, 1.02)  & 17.15 (67.04, 1.05)  & 27.71 (41.49, 0.65)  &  27.93 (41.16, 0.64)  & 26.27 (43.77, 0.68)  &  19 
\hline
Satellite7  & n/a     & 502.51 (n/a, n/a)    & 468.07 (n/a, n/a)    & 370.43 (n/a, n/a)    &  375.86 (n/a, n/a)    & 351.69 (n/a, n/a)    &  21 
\hline
ZenoTrav11  & 546.67  & 16.58 (32.97, 0.52)  & 15.64 (34.95, 0.55)  & 15.29 (35.75, 0.56)  &  14.71 (37.16, 0.58)  & 14.41 (37.94, 0.59)  &  14 
\hline
PipesNoTk24 & 1396.29 & 40.34 (34.61, 0.54)  & 39.85 (35.04, 0.55)  & 38.08 (36.67, 0.57)  &  35.34 (39.51, 0.62)  & 34.53 (40.44, 0.63)  &  24 
\hline
Pegsol28    & 1010.65 & 21.77 (46.42, 0.73)  & 21.31 (47.43, 0.74)  & 20.75 (48.71, 0.76)  &  20.47 (49.37, 0.77)  & 19.64 (51.46, 0.80)  &  35 
\hline
Sokoban24   & 2635.37 & 57.29 (46.00, 0.72)  & 51.82 (50.86, 0.79)  & 50.99 (51.68, 0.81)  &  48.08 (54.81, 0.86)  & 46.51 (56.66, 0.89)  &  205 
\hline

Speedups (64 cores, with dummy processes)
            & 1 core  & 64 cores (4 nodes)   & 64 cores (8 nodes)   & 64 cores (16 nodes)  & 64 cores (32 nodes)  & 64 cores (64 nodes)  & Opt. plan Len.
Freecell7   & 2864.64 & 66.85 (42.85, 0.67)  & 70.59 (40.58, 0.63)  & 72.13 (39.71, 0.62)  & 77.49 (36.97, 0.58)  & 76.15 (37.62, 0.59)  &  41 
\hline
Rover12     & 1149.74 & 17.68 (65.03, 1.02)  & 35.07 (32.78, 0.51)  & 19.30 (59.57, 0.93)  & 34.47 (33.35, 0.52)  & 34.98 (32.87, 0.51)  &  19 
\hline
Satellite7  & n/a     & 502.51 (n/a, n/a)    & 466.16 (n/a, n/a)    & 535.86 (n/a, n/a)    & 445.64 (n/a, n/a)    & 462.22 (n/a, n/a)    &  21 
\hline
ZenoTrav11  & 546.67  & 16.58 (32.97, 0.52)  & 21.17 (25.82, 0.40)  & 20.15 (27.13, 0.42)  & 19.89 (27.48, 0.43)  & 20.54 (26.61, 0.42)  &  14 
\hline
PipesNoTk24 & 1396.29 & 40.34 (34.61, 0.54)  & 44.99 (31.04, 0.48)  & 45.26 (30.85, 0.48)  & 43.79 (31.89, 0.50)  & 43.80 (31.88, 0.50)  &  24 
\hline
Pegsol28    & 1010.65 & 21.77 (46.42, 0.73)  & 22.88 (44.17, 0.69)  & n/a                  & 23.23 (43.51, 0.68)  & 23.44 (43.12, 0.67)  &  35 
\hline
Sokoban24   & 2635.37 & 57.29 (46.00, 0.72)  & 57.45 (45.87, 0.72)  & 56.07 (47.00, 0.73)  & 57.92 (45.50, 0.71)  & 57.16 (46.11, 0.72)  &  205 
\hline

Speedups (16 cores, abst=5000)
             & 1 core  & 16 cores (1 node)     & Abstraction init. time & Opt. plan Len.
Driverslog13 & 29.88 &  2.87 (10.41, 0.65)     & 1.96                   & 36 
\hline
Rover12      & 468.56 &  49.55 (9.46, 0.59)    & 3.50                   & 19 
\hline
ZenoTrav11   & 13.50 &  1.35 (10.00, 0.62)     & 1.31                   & 14 
\hline
PipesNoTk24  & 178.67 &  16.20 (11.03, 0.69)   & 23.19                  & 24 
\hline
Sokoban24    & 1429.95 &  114.37 (12.50, 0.78) & 4.07                   & 205 
\hline

# of problems solved in opt sokoban (30 problems)
sequential (32GB) 22
512 cores (1TB)   28
1024 cores (2TB)  28


Speedups (64-1024 cores, 24 puzzle)
    & 1 core  & 64 cores (4 nodes)  & 128 cores (8 nodes)  & 512 cores (32 nodes)  & 1024 cores (64 nodes) & opt. plan len.
P1  & 842.03  & 35.00 (24.06, 0.38) &  22.11 (38.08, 0.30) &  8.23 (102.31, 0.20)  &  16.27 (51.75, 0.05)  &  95 
P29 & 1154.42 & 41.10 (28.09, 0.44) &  22.84 (50.54, 0.39) &  10.61 (108.81, 0.21) &  18.74 (61.60, 0.06)  &  88 

Search Overhead (64-1024 cores, 24 puzzle) 
    &   1 core        & 64 cores (4 nodes) & 128 cores (8 nodes) & 512 cores (32 nodes)  & 1024 cores (64 nodes)
P1  &  120901818 (-)  &  166881300 (38.03\%) &  222242508 (83.82\%) &  279681479 (131.33\%) &  1033699414 (754.99\%)
P29 &  160409172 (-)  &  212973518 (32.77\%) &  224665656 (40.06\%) &  395710212 (146.69\%) &  1375155895 (757.28\%) 

# of problems solved in Korf's instances (50 problems)
sequential (32GB)  2
512 cores (1TB)   21
1024 cores (2TB)  15 
Korf's IDA*       50



==> unused_fungate_results.tex <==
Speedups (1-8 cores)
            & 1 core & HDA*(4 cores)       & PRA*(4 cores)       & WSA* (4 cores)      & HDA* (8 cores)       & PRA* (8 cores)     & WSA* (8 cores)      & Abst. time & Opt. plan Len.
Depot4      & 73.34  & 29.70 (2.47, 0.62)  & 39.07 (1.88, 0.47)  & 34.12 (2.15, 0.54)  & 15.79 (4.64, 0.58)  & 21.18 (3.46, 0.43)  & 19.40 (3.78, 0.47)  &  3.56 & 30 
\hline
Driverlog8  & 85.79  & 39.72 (2.16, 0.54)  & 56.57 (1.52, 0.38)  & 48.94 (1.75, 0.44)  & 20.74 (4.14, 0.52)  & 34.03 (2.52, 0.32)  & 30.21 (2.84, 0.35)  &  0.15 & 22 
\hline
Freecell5   & 143.57 & 47.41 (3.03, 0.76)  & 56.24 (2.55, 0.64)  & 52.32 (2.74, 0.69)  & 24.90 (5.77, 0.72)  & 30.84 (4.66, 0.58)  & 27.67 (5.19, 0.65)  &  8.17 & 30 
\hline
Rover12     & 517.67 & 221.61 (2.34, 0.58) & 286.31 (1.81, 0.45) & 256.31 (2.02, 0.50) & 117.27 (4.41, 0.55) & 162.18 (3.19, 0.40) & 145.90 (3.55, 0.44) &  1.03 & 19 
\hline
ZenoTrav9   & 170.61 & 75.65 (2.26, 0.56)  & 113.96 (1.50, 0.37) & 92.82 (1.84, 0.46)  & 40.90 (4.17, 0.52)  & 66.61 (2.56, 0.32)  & 57.99 (2.94, 0.37)  &  0.19 & 21 
\hline
PipesNoTk14 & 201.52 & 71.79 (2.81, 0.70)  & 96.90 (2.08, 0.52)  & 87.60 (2.30, 0.58)  & 38.23 (5.27, 0.66)  & 58.35 (3.45, 0.43)  & 53.69 (3.75, 0.47)  &  1.70 & 30 
\hline
PipesTk15   & 81.26  & 27.19 (2.99, 0.75)  & 36.83 (2.21, 0.55)  & 32.59 (2.49, 0.62)  & 15.00 (5.42, 0.68)  & 21.02 (3.87, 0.48)  & 19.03 (4.27, 0.53)  &  7.31 & 30 
\hline
Pegsol28    & 837.78 & 269.10 (3.11, 0.78) & 370.04 (2.26, 0.57) & 335.10 (2.50, 0.63) & 138.47 (6.05, 0.76) & 233.29 (3.59, 0.45) & 215.04 (3.90, 0.49) &  0.64 & 35 
\hline
Sokoban22   & 474.75 & 149.46 (3.18, 0.79) & 195.49 (2.43, 0.61) & 180.50 (2.63, 0.66) & 77.82 (6.10, 0.76)  & 115.80 (4.10, 0.51) & 106.60 (4.45, 0.56) &  2.23 & 172 
\hline


Depot10     & 484.74 & 227.54 (2.13, 0.53) & 292.32 (1.66, 0.41) & 240.81 (2.01, 0.50) & 127.59 (3.80, 0.47) & 152.97 (3.17, 0.40) & 127.50 (3.80, 0.48) &  2.14 & 24 
\hline
Pegsol26    & 57.01  & 18.95 (3.01, 0.75)  & 27.72 (2.06, 0.51)  & 25.41 (2.24, 0.56)  & 10.01 (5.70, 0.71)  & 17.63 (3.23, 0.40)  & 16.88 (3.38, 0.42)  &  9.29 & 27 
\hline
Pegsol27    & 192.74 & 62.29 (3.09, 0.77)  & 87.78 (2.20, 0.55)  & 80.45 (2.40, 0.60)  & 32.15 (6.00, 0.75)  & 55.53 (3.47, 0.43)  & 52.42 (3.68, 0.46)  &  1.08 & 28 
\hline
Sokoban5    & 200.45 & 56.79 (3.53, 0.88)  & 65.54 (3.06, 0.76)  & 84.36 (2.38, 0.59)  & 34.02 (5.89, 0.74)  & 49.92 (4.02, 0.50)  & 41.72 (4.80, 0.60)  &  6.53 & 25 
\hline
Sokoban8    & 83.84  & 29.59 (2.83, 0.71)  & 39.42 (2.13, 0.53)  & 36.31 (2.31, 0.58)  & 14.94 (5.61, 0.70)  & 24.39 (3.44, 0.43)  & 22.18 (3.78, 0.47)  &  0.73 & 76 
\hline
Sokoban15   & 198.71 & 62.03 (3.20, 0.80)  & 82.44 (2.41, 0.60)  & 77.00 (2.58, 0.65)  & 32.26 (6.16, 0.77)  & 49.98 (3.98, 0.50)  & 48.08 (4.13, 0.52)  &  0.48 & 244 
\hline
Sokoban18   & 57.67  & 18.16 (3.18, 0.79)  & 24.83 (2.32, 0.58)  & 23.51 (2.45, 0.61)  & 9.60 (6.01, 0.75)   & 15.14 (3.81, 0.48)  & 14.42 (4.00, 0.50)  &  0.64 & 197 
\hline
Sokoban19   & 176.66 & 58.42 (3.02, 0.76)  & 81.49 (2.17, 0.54)  & 73.97 (2.39, 0.60)  & 31.71 (5.57, 0.70)  & 49.42 (3.57, 0.45)  & 45.39 (3.89, 0.49)  &  1.46 & 164 
\hline 


==> uused_tsubame_results.tex <==
Speedups (16-512 cores) 
            1 core     & 16 cores (1 node)     & 64 cores (4 nodes)    & 128 cores (8 nodes)    & 512 cores (32 nodes)  & Abstraction init. time & Opt. plan Len.
Depot13     & 328.04   &  35.82 (9.16, 0.57)   &  19.15 (17.13, 0.27)  &  5.47 (59.97, 0.47)    &  13.80 (23.77, 0.05)  &  6.13                  & 25 
\hline
Driverlog13 & n/a      &  n/a (n/a, n/a)       &  n/a (n/a, n/a)       &  n/a (n/a, n/a)        &  41.01 (n/a, n/a)     &  0.58                  & 26 
\hline
Freecell6   & n/a      &  n/a (n/a, n/a)       &  n/a (n/a, n/a)       &  137.08 (n/a, n/a)     &  50.36 (n/a, n/a)     &  7.80                  & 34 
\hline
Freecell7   & 2864.64  &  n/a (n/a, n/a)       &  66.85 (42.85, 0.67)  &  34.00 (84.25, 0.66)   &  11.59 (247.16, 0.48) &  9.71                  & 41 
\hline
Rover6      & 9291.32  &  n/a (n/a, n/a)       &  171.58 (54.15, 0.85) &  67.28 (138.10, 1.08)  &  17.18 (540.82, 1.06) &  0.16                  & 36 
\hline
Rover12     & 1149.74  &  109.62 (10.49, 0.66) &  17.68 (65.03, 1.02)  &  14.50 (79.29, 0.62)   &  4.06 (283.19, 0.55)  &  0.16                  & 19 
\hline
Satellite7  & n/a      &  n/a (n/a, n/a)       &  502.51 (n/a, n/a)    &  209.73 (n/a, n/a)     &  55.31 (n/a, n/a)     &  0.31                  & 21 
\hline
ZenoTrav11  & 546.67   &  61.26 (8.92, 0.56)   &  16.58 (32.97, 0.52)  &  8.55 (63.94, 0.50)    &  2.76 (198.07, 0.39)  &  0.32                  & 14 
\hline
ZenoTrav12  & n/a      &  n/a (n/a, n/a)       &  n/a (n/a, n/a)       &  n/a (n/a, n/a)        &  180.80 (n/a, n/a)    &  0.44                  & 21 
\hline
PipesNoTk24 & 1396.29  &  139.25 (10.03, 0.63) &  40.34 (34.61, 0.54)  &  20.47 (68.21, 0.53)   &  6.11 (228.52, 0.45)  &  6.68                  & 24 
\hline
Pegsol28    & 1010.65  &  83.22 (12.14, 0.76)  &  21.77 (46.42, 0.73)  &  10.41 (97.08, 0.76)   &  3.23 (312.90, 0.61)  &  0.96                  & 35 
\hline
Pegsol29    & 5143.24  &  n/a (n/a, n/a)       &  n/a (n/a, n/a)       &  52.28 (98.38, 0.77)   &  13.86 (371.09, 0.72) &  15.47                 & 37 
\hline
Pegsol30    & n/a      &  n/a (n/a, n/a)       &  n/a (n/a, n/a)       &  n/a (n/a, n/a)        &  34.14 (n/a, n/a)     &  3.05                  & 48 
\hline
Sokoban24   & 2635.37  &  n/a (n/a, n/a)       &  57.29 (46.00, 0.72)  &  33.52 (78.62, 0.61)   &  15.97 (165.02, 0.32) &  1.43                  & 205 
\hline
Sokoban25   & 2952.19  &  n/a (n/a, n/a)       &  71.49 (41.30, 0.65)  &  37.68 (78.35, 0.61)   &  16.24 (181.79, 0.36) &  2.29                  & 155 
\hline
Sokoban26   & n/a      &  n/a (n/a, n/a)       &  155.20 (n/a, n/a)    &  77.60 (n/a, n/a)      &  25.29 (n/a, n/a)     &  2.16                  & 135 
\hline
Sokoban27   & n/a      &  n/a (n/a, n/a)       &  n/a (n/a, n/a)       &  n/a (n/a, n/a)        &  36.53 (n/a, n/a)     &  3.40                  & 87 
\hline
Sokoban28   & 2582.16  &  n/a (n/a, n/a)       &  65.91 (39.18, 0.61)  &  33.39 (77.33, 0.60)   &  14.43 (178.94, 0.35) &  1.21                  & 135 
\hline

Search Overhead (16-512 cores)
               1 core        & 16 cores (1 node)   & 64 cores (4 nodes)   & 128 cores (8 nodes)   & 512 cores (32 nodes)  & Opt. plan Len.
Depot13     &  10862511 (-)  &  10867719 (0.05\%)  &  21150502 (94.71\%)  &  11385211 (4.81\%)    &  13917296 (28.12\%)   &  25 
\hline
Driverlog13 &  n/a (-)       &  n/a (n/a)          &  n/a (n/a)           &  n/a (n/a)            &  625188136 (n/a)      &  26 
\hline
Freecell6   &  n/a (-)       &  n/a (n/a)          &  n/a (n/a)           &  337534088 (n/a)      &  512715407 (n/a)      &  34 
\hline
Freecell7   &  92584775 (-)  &  n/a (n/a)          &  94375606 (1.93\%)   &  95500727 (3.15\%)    &  117518741 (26.93\%)  &  41 
\hline
Rover6      &  221406982 (-) &  n/a (n/a)          &  285421179 (28.91\%) &  222408052 (0.45\%)   &  223627845 (1.00\%)   &  36 
\hline
Rover12     &  37243958 (-)  &  37307482 (0.17\%)  &  23230170 (-37.63\%) &  37443936 (0.54\%)    &  37561310 (0.85\%)    &  19 
\hline
Satellite7  &  n/a (-)       &  n/a (n/a)          &  222759213 (n/a)     &  191082376 (n/a)      &  187116616 (n/a)      &  21 
\hline
ZenoTrav11  &  14619024 (-)  &  14619585 (0.00\%)  &  14637721 (0.13\%)   &  14740958 (0.83\%)    &  15724503 (7.56\%)    &  14 
\hline
ZenoTrav12  &  n/a (-)       &  n/a (n/a)          &  n/a (n/a)           &  n/a (n/a)            &  1185737053 (n/a)     &  21 
\hline
PipesNoTk24 &  72782203 (-)  &  72805219 (0.03\%)  &  72836410 (0.07\%)   &  73260029 (0.66\%)    &  75243695 (3.38\%)    &  24 
\hline
Pegsol28    &  111419815 (-) &  114198633 (2.49\%) &  113524270 (1.89\%)  &  114337541 (2.62\%)   &  118067547 (5.97\%)   &  35 
\hline
Pegsol29    &  478930258 (-) &  n/a (n/a)          &  n/a (n/a)           &  499041168 (4.20\%)   &  501172298 (4.64\%)   &  37 
\hline
Pegsol30    &  n/a (-)       &  n/a (n/a)          &  n/a (n/a)           &  n/a (n/a)            &  1405030332 (n/a)     &  48 
\hline
Sokoban24   &  241797086 (-) &  n/a (n/a)          &  278360621 (15.12\%) &  356505847 (47.44\%)  &  597653466 (147.17\%) &  205 
\hline
Sokoban25   &  308789201 (-) &  n/a (n/a)          &  332240874 (7.59\%)  &  349230333 (13.10\%)  &  609713989 (97.45\%)  &  155 
\hline
Sokoban26   &  n/a (-)       &  n/a (n/a)          &  720848950 (n/a)     &  760380596 (n/a)      &  973650946 (n/a)      &  135 
\hline
Sokoban27   &  n/a (-)       &  n/a (n/a)          &  n/a (n/a)           &  n/a (n/a)            &  1359144655 (n/a)     &  87 
\hline
Sokoban28   &  263787718 (-) &  n/a (n/a)          &  309092631 (17.17\%) &  312008346 (18.28\%)  &  537206211 (103.65\%) &  135 
\hline

Speedups (64 cores, real) 
               1 core & 64 cores (4 nodes)    & 64 cores (8 nodes)    & 64 cores (16 nodes)   & 64 cores (32 nodes)   & 64 cores (64 nodes) & Opt. plan Len.
Depot13     & 328.04  &  19.15 (17.13, 0.27)  &  18.55 (17.68, 0.28)  &  17.40 (18.85, 0.29)  &  8.86 (37.03, 0.58)   &  xxx                & 25 
\hline
Freecell7   & 2864.64 &  66.85 (42.85, 0.67)  &  68.61 (41.75, 0.65)  &  64.29 (44.56, 0.70)  &  59.24 (48.36, 0.76)  &  xxx                & 41 
\hline
Rover6      & 9291.32 &  171.58 (54.15, 0.85) &  169.46 (54.83, 0.86) &  127.35 (72.96, 1.14) &  124.69 (74.52, 1.16) &  xxx                & 36 
\hline
Rover12     & 1149.74 &  17.68 (65.03, 1.02)  &  17.15 (67.04, 1.05)  &  27.71 (41.49, 0.65)  &  27.93 (41.16, 0.64)  &  xxx                & 19 
\hline
Satellite7  & n/a     &  502.51 (n/a, n/a)    &  468.07 (n/a, n/a)    &  370.43 (n/a, n/a)    &  375.86 (n/a, n/a)    &  xxx                & 21 
\hline
ZenoTrav11  & 546.67  &  16.58 (32.97, 0.52)  &  15.64 (34.95, 0.55)  &  15.29 (35.75, 0.56)  &  14.71 (37.16, 0.58)  &  xxx                & 14 
\hline
PipesNoTk24 & 1396.29 &  40.34 (34.61, 0.54)  &  39.85 (35.04, 0.55)  &  38.08 (36.67, 0.57)  &  35.34 (39.51, 0.62)  &  xxx                & 24 
\hline
Pegsol28    & 1010.65 &  21.77 (46.42, 0.73)  &  21.31 (47.43, 0.74)  &  20.75 (48.71, 0.76)  &  20.47 (49.37, 0.77)  &  xxx                & 35 
\hline
Sokoban24   & 2635.37 &  57.29 (46.00, 0.72)  &  51.82 (50.86, 0.79)  &  50.99 (51.68, 0.81)  &  48.08 (54.81, 0.86)  &  xxx                & 205 
\hline
Sokoban25   & 2952.19 &  71.49 (41.30, 0.65)  &  66.12 (44.65, 0.70)  &  65.22 (45.27, 0.71)  &  62.43 (47.29, 0.74)  &  xxx                & 155 
\hline
Sokoban28   & 2582.16 &  65.91 (39.18, 0.61)  &  61.02 (42.32, 0.66)  &  57.45 (44.95, 0.70)  &  55.26 (46.73, 0.73)  &  xxx                & 135 
\hline

Speedups (64 cores with dummy processes)
             1 core   & 64 cores (4 nodes)    &  64 cores (8 nodes)   & 64 cores (16 nodes)   & 64 cores (32 nodes)   & 64 cores (64 nodes) & Opt. plan Len.
Depot13     & 328.04  &  19.15 (17.13, 0.27)  &  11.69 (28.06, 0.44)  &  20.55 (15.96, 0.25)  &  11.25 (29.16, 0.46)  &  xxx                & 25 
\hline
Freecell7   & 2864.64 &  66.85 (42.85, 0.67)  &  70.59 (40.58, 0.63)  &  72.13 (39.71, 0.62)  &  77.49 (36.97, 0.58)  &  xxx                & 41 
\hline
Rover6      & 9291.32 &  171.58 (54.15, 0.85) &  146.94 (63.23, 0.99) &  191.38 (48.55, 0.76) &  150.14 (61.88, 0.97) &  xxx                & 36 
\hline
Rover12     & 1149.74 &  17.68 (65.03, 1.02)  &  35.07 (32.78, 0.51)  &  19.30 (59.57, 0.93)  &  34.47 (33.35, 0.52)  &  xxx                & 19 
\hline
Satellite7  & n/a     &  502.51 (n/a, n/a)    &  466.16 (n/a, n/a)    &  535.86 (n/a, n/a)    &  445.64 (n/a, n/a)    &  xxx                & 21 
\hline
ZenoTrav11  & 546.67  &  16.58 (32.97, 0.52)  &  21.17 (25.82, 0.40)  &  20.15 (27.13, 0.42)  &  19.89 (27.48, 0.43)  &  xxx                & 14 
\hline
PipesNoTk24 & 1396.29 &  40.34 (34.61, 0.54)  &  44.99 (31.04, 0.48)  &  45.26 (30.85, 0.48)  &  43.79 (31.89, 0.50)  &  xxx                & 24 
\hline
Pegsol28    & 1010.65 &  21.77 (46.42, 0.73)  &  22.88 (44.17, 0.69)  &  n/a (n/a, n/a)       &  23.23 (43.51, 0.68)  &  xxx                & 35 
\hline
Sokoban24   & 2635.37 &  57.29 (46.00, 0.72)  &  57.45 (45.87, 0.72)  &  56.07 (47.00, 0.73)  &  57.92 (45.50, 0.71)  &  xxx                & 205 
\hline
Sokoban25   & 2952.19 &  71.49 (41.30, 0.65)  &  77.94 (37.88, 0.59)  &  71.75 (41.15, 0.64)  &  74.07 (39.86, 0.62)  &  xxx                & 155 
\hline
Sokoban28   & 2582.16 &  65.91 (39.18, 0.61)  &  62.96 (41.01, 0.64)  &  64.95 (39.76, 0.62)  &  64.82 (39.84, 0.62)  &  xxx                & 135 
\hline

Speedups (16 cores, abst size=5000)
             1 core     & 16 cores (1 node)     & Abstraction init. time & Opt. plan Len.
Depot13      & 41.08    &  2.95 (13.93, 0.87)   &  18.92                 & 25 
\hline
Driverslog13 & 29.88    &  2.87 (10.41, 0.65)   &  1.81                  & 36 
\hline
Rover6       & 2152.50  &  192.71 (11.17, 0.70) &  0.74                  & 36 
\hline
Rover12      & 468.56   &  49.55 (9.46, 0.59)   &  3.23                  & 19 
\hline
ZenoTrav11   & 13.50    &  1.35 (10.00, 0.62)   &  1.21                  & 14 
\hline
PipesNoTk24  & 178.67   &  16.20 (11.03, 0.69)  &  21.41                 & 24 
\hline
Sokoban24    & 1429.95  &  114.37 (12.50, 0.78) &  3.76                  & 205 
\hline

\# of problems solved in opt sokoban (30 problems)
sequential (32GB) 22
512 cores (1TB)   28

Speedups (64-512 cores, 24 puzzle) 
    & 1 core  & 64 cores (4 nodes)   & 128 cores (8 nodes)  & 512 cores (32 nodes)  & opt. plan len.
P1  & 842.03  &  35.00 (24.06, 0.38) &  22.11 (38.08, 0.30) &  8.23 (102.31, 0.20)  &  95 
P29 & 1154.42 &  41.10 (28.09, 0.44) &  22.84 (50.54, 0.39) &  10.61 (108.81, 0.21) &  88 

Search Overhead (64-512 cores, 24 puzzle) 
    &   1 core        & 64 cores (4 nodes)   & 128 cores (8 nodes)  & 512 cores (32 nodes) 
P1  &  120901818 (-)  &  166881300 (38.03\%) &  222242508 (83.82\%) &  279681479 (131.33\%)
P29 &  160409172 (-)  &  212973518 (32.77\%) &  224665656 (40.06\%) &  395710212 (146.69\%)


# of problems solved in Korf's instances (50 problems)
sequential (32GB)  2
512 cores (1TB)   21

